(704) Interamnia: A transitional object between a dwarf planet and a typical irregular-shaped minor body

With an estimated diameter in the 320 to 350 km range, (704) Interamnia is the fifth largest main belt asteroid and one of the few bodies that fills the gap in size between the four largest bodies with $D$ > 400 km (Ceres, Vesta, Pallas and Hygiea) and the numerous smaller bodies with $D$ $\lesssim$ 200 km. However, despite its large size, little is known about the shape and spin state of Interamnia and, therefore, about its bulk composition and past collisional evolution. We aimed to test at what size and mass the shape of a small body departs from a nearly ellipsoidal equilibrium shape (as observed in the case of the four largest asteroids) to an irregular shape as routinely observed in the case of smaller ($D$ $\lesssim$ 200 km) bodies. We observed Interamnia as part of our ESO VLT/SPHERE large program (ID: 199.C-0074) at thirteen different epochs. In addition, several new optical lightcurves were recorded. These data, along with stellar occultation data from the literature, were fed to the All-Data Asteroid Modeling (ADAM) algorithm to reconstruct the 3D-shape model of Interamnia and to determine its spin state. Interamnia's volume-equivalent diameter of 332 $\pm$ 6 km implies a bulk density of $\rho$=1.98 $\pm$ 0.68 gcm$^{-3}$ , which suggests that Interamnia - like Ceres and Hygiea - contains a high fraction of water ice, consistent with the paucity of apparent craters. Our observations reveal a shape that can be well approximated by an ellipsoid, and that is compatible with a fluid hydrostatic equilibrium at the 2 $\sigma$ level. The rather regular shape of Interamnia implies that the size and mass limit, under which the shapes of minor bodies with a high amount of water ice in the subsurface become irregular, has to be searched among smaller ($D$ $\lesssim$ 300km) less massive ($m$ $\lesssim$ 3x10$^{19}$ kg) bodies.

==> tabs/tab_ao.tex <==
%\scriptsize{
\begin{table*}
\caption{\label{tab:ao}List of VLT/SPHERE disk-resolved images obtained in the I filter by the ZIMPOL camera. For each observation, the table gives the epoch, the exposure time, the airmass, the distance to the Earth $\Delta$ and the Sun $r$, the phase angle $\alpha$, and the angular diameter $D_\mathrm{a}$.}
\centering
\begin{tabular}{rr rr rrr r}
\hline 
\multicolumn{1}{c} {Date} & \multicolumn{1}{c} {UT} & \multicolumn{1}{c} {Exp} & \multicolumn{1}{c} {Airmass} & \multicolumn{1}{c} {$\Delta$} & \multicolumn{1}{c} {$r$} & \multicolumn{1}{c} {$\alpha$} & \multicolumn{1}{c} {$D_\mathrm{a}$} \\
\multicolumn{1}{c} {} & \multicolumn{1}{c} {} & \multicolumn{1}{c} {(s)} & \multicolumn{1}{c} {} & \multicolumn{1}{c} {(AU)} & \multicolumn{1}{c} {(AU)} & \multicolumn{1}{c} {(\degr)} & \multicolumn{1}{c} {(\arcsec)} \\
% &  &  &  &  &  &  &  & &  \\
\hline\hline
  2017-07-14 &      8:57:06 & 200 & 1.46 & 2.24 & 2.62 & 22.4 & 0.203 \\
  2017-07-14 &      9:07:35 & 200 & 1.45 & 2.24 & 2.62 & 22.4 & 0.203 \\
  2017-08-29 &      5:39:04 & 200 & 1.71 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      5:42:36 & 200 & 1.70 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      5:46:06 & 200 & 1.70 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      5:49:35 & 200 & 1.69 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      5:53:04 & 200 & 1.69 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      7:51:55 & 200 & 1.88 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      7:55:24 & 200 & 1.89 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      7:58:55 & 200 & 1.91 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      8:02:25 & 200 & 1.93 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-08-29 &      8:05:53 & 200 & 1.95 & 1.78 & 2.60 & 15.9 & 0.256 \\
  2017-09-02 &      5:21:35 & 200 & 1.72 & 1.76 & 2.60 & 15.0 & 0.259 \\
  2017-09-02 &      5:25:05 & 200 & 1.71 & 1.76 & 2.60 & 15.0 & 0.259 \\
  2017-09-02 &      5:28:35 & 200 & 1.71 & 1.76 & 2.60 & 15.0 & 0.259 \\
  2017-09-02 &      5:32:05 & 200 & 1.70 & 1.76 & 2.60 & 15.0 & 0.259 \\
  2017-09-02 &      5:35:33 & 200 & 1.70 & 1.76 & 2.60 & 15.0 & 0.259 \\
  2017-09-04 &      6:28:32 & 200 & 1.72 & 1.74 & 2.60 & 14.5 & 0.261 \\
  2017-09-04 &      6:32:03 & 200 & 1.73 & 1.74 & 2.60 & 14.5 & 0.261 \\
  2017-09-04 &      6:35:34 & 200 & 1.73 & 1.74 & 2.60 & 14.5 & 0.261 \\
  2017-09-04 &      6:39:03 & 200 & 1.74 & 1.74 & 2.60 & 14.5 & 0.261 \\
  2017-09-04 &      6:42:32 & 200 & 1.75 & 1.74 & 2.60 & 14.5 & 0.261 \\
  2017-09-05 &      7:18:13 & 200 & 1.89 & 1.74 & 2.60 & 14.3 & 0.261 \\
  2017-09-05 &      7:21:43 & 200 & 1.91 & 1.74 & 2.60 & 14.3 & 0.261 \\
  2017-09-05 &      7:25:13 & 200 & 1.92 & 1.74 & 2.60 & 14.3 & 0.261 \\
  2018-12-19 &      6:09:44 & 147 & 1.35 & 2.15 & 3.02 & 10.1 & 0.212 \\
  2018-12-19 &      6:12:22 & 147 & 1.35 & 2.15 & 3.02 & 10.1 & 0.212 \\
  2018-12-19 &      6:15:01 & 147 & 1.34 & 2.15 & 3.02 & 10.1 & 0.212 \\
  2018-12-19 &      6:17:38 & 147 & 1.34 & 2.15 & 3.02 & 10.1 & 0.212 \\
  2018-12-19 &      6:20:16 & 147 & 1.34 & 2.15 & 3.02 & 10.1 & 0.212 \\
  2018-12-22 &      5:23:49 & 147 & 1.41 & 2.13 & 3.03 & 9.2 & 0.214 \\
  2018-12-22 &      5:26:28 & 147 & 1.40 & 2.13 & 3.03 & 9.2 & 0.214 \\
  2018-12-22 &      5:29:07 & 147 & 1.39 & 2.13 & 3.03 & 9.2 & 0.214 \\
  2018-12-22 &      5:31:44 & 147 & 1.39 & 2.13 & 3.03 & 9.2 & 0.214 \\
  2018-12-22 &      5:34:22 & 147 & 1.38 & 2.13 & 3.03 & 9.2 & 0.214 \\
  2018-12-29 &      4:37:47 & 147 & 1.43 & 2.10 & 3.04 & 6.7 & 0.217 \\
  2018-12-29 &      4:40:26 & 147 & 1.43 & 2.10 & 3.04 & 6.7 & 0.217 \\
  2018-12-29 &      4:43:04 & 147 & 1.42 & 2.10 & 3.04 & 6.7 & 0.217 \\
  2018-12-29 &      4:45:42 & 147 & 1.41 & 2.10 & 3.04 & 6.7 & 0.217 \\
  2018-12-29 &      4:48:19 & 147 & 1.40 & 2.10 & 3.04 & 6.7 & 0.217 \\
  2019-01-08 &      3:04:48 & 147 & 1.60 & 2.08 & 3.05 & 3.3 & 0.219 \\
  2019-01-08 &      3:07:27 & 147 & 1.59 & 2.08 & 3.05 & 3.3 & 0.219 \\
  2019-01-08 &      3:10:05 & 147 & 1.58 & 2.08 & 3.05 & 3.3 & 0.219 \\
  2019-01-08 &      3:12:43 & 147 & 1.56 & 2.08 & 3.05 & 3.3 & 0.219 \\
  2019-01-08 &      3:15:21 & 147 & 1.55 & 2.08 & 3.05 & 3.3 & 0.219 \\
  2019-01-09 &      6:40:27 & 147 & 1.42 & 2.08 & 3.05 & 2.9 & 0.219 \\
  2019-01-09 &      6:43:05 & 147 & 1.43 & 2.08 & 3.05 & 2.9 & 0.219 \\
  2019-01-09 &      6:45:44 & 147 & 1.44 & 2.08 & 3.05 & 2.9 & 0.219 \\
  2019-01-09 &      6:48:22 & 147 & 1.44 & 2.08 & 3.05 & 2.9 & 0.219 \\
  2019-01-09 &      6:51:00 & 147 & 1.45 & 2.08 & 3.05 & 2.9 & 0.219 \\
  2019-01-10 &      7:19:31 & 147 & 1.59 & 2.08 & 3.06 & 2.6 & 0.219 \\
  2019-01-10 &      7:22:07 & 147 & 1.61 & 2.08 & 3.06 & 2.6 & 0.219 \\
  2019-01-10 &      7:24:47 & 147 & 1.62 & 2.08 & 3.06 & 2.6 & 0.219 \\
  2019-01-10 &      7:27:23 & 147 & 1.64 & 2.08 & 3.06 & 2.6 & 0.219 \\
  2019-01-10 &      7:30:00 & 147 & 1.65 & 2.08 & 3.06 & 2.6 & 0.219 \\
  2019-01-14 &      6:43:25 & 147 & 1.51 & 2.08 & 3.06 & 2.0 & 0.219 \\
  2019-01-14 &      6:46:03 & 147 & 1.52 & 2.08 & 3.06 & 2.0 & 0.219 \\
  2019-01-14 &      6:48:40 & 147 & 1.53 & 2.08 & 3.06 & 2.0 & 0.219 \\
  2019-01-14 &      6:51:17 & 147 & 1.55 & 2.08 & 3.06 & 2.0 & 0.219 \\
  2019-01-14 &      6:53:53 & 147 & 1.56 & 2.08 & 3.06 & 2.0 & 0.219 \\
\hline
\end{tabular}
%\tablefoot{
%    Notes...
%    }
\end{table*}


==> tabs/tab_lcs.tex <==
\onecolumn
%\scriptsize{
\begin{longtable}{rlr rrr l l}
\caption{\label{tab:lcs}List of optical disk-integrated lightcurves used for \adam{} shape modeling. For each lightcurve, the table gives the epoch, the number of individual measurements $N_p$, asteroid's distances to the Earth $\Delta$ and the Sun $r$, phase angle $\varphi$, photometric filter and observation information.}\\
\hline 
\multicolumn{1}{c} {N} & \multicolumn{1}{c} {Epoch} & \multicolumn{1}{c} {$N_p$} & \multicolumn{1}{c} {$\Delta$} & \multicolumn{1}{c} {$r$} & \multicolumn{1}{c} {$\varphi$} & \multicolumn{1}{c} {Filter} & Reference \\
 &  &  & (AU) & (AU) & (\degr) &  &  \\
\hline\hline
\endfirsthead
\caption{continued.}\\
\hline
\multicolumn{1}{c} {N} & \multicolumn{1}{c} {Epoch} & \multicolumn{1}{c} {$N_p$} & \multicolumn{1}{c} {$\Delta$} & \multicolumn{1}{c} {$r$} & \multicolumn{1}{c} {$\varphi$} & \multicolumn{1}{c} {Filter} & Reference \\
 &  &  & (AU) & (AU) & (\degr) &  &  \\
\hline\hline
\endhead
\hline
\endfoot
\hline
     1	  &  1964-11-22.7  &  81    &  1.82  &  2.75  &  8.1   &  V &  \citet{Yang1965} \\
     2	  &  1964-11-23.7  &  57    &  1.81  &  2.75  &  7.7   &  V &  \citet{Yang1965} \\
     3	  &  1969-08-16.5  &  8     &  2.18  &  2.58  &  22.6  &  V &  \citet{Tempesti1975} \\
     4	  &  1969-08-20.6  &  7     &  2.14  &  2.58  &  22.3  &  V &  \citet{Tempesti1975} \\
     5	  &  1969-08-21.5  &  12    &  2.13  &  2.58  &  22.2  &  V &  \citet{Tempesti1975} \\
     6	  &  1969-09-08.5  &  12    &  1.95  &  2.59  &  19.9  &  V &  \citet{Tempesti1975} \\
     7	  &  1969-10-05.6  &  13    &  1.74  &  2.60  &  13.9  &  V &  \citet{Tempesti1975} \\
     8	  &  1969-10-15.4  &  10    &  1.70  &  2.60  &  11.4  &  V &  \citet{Tempesti1975} \\
     9	  &  1969-11-01.4  &  11    &  1.68  &  2.61  &  9.1   &  V &  \citet{Tempesti1975} \\
    10	  &  1969-11-03.4  &  15    &  1.68  &  2.61  &  9.2   &  V &  \citet{Tempesti1975} \\
    11	  &  1969-11-10.5  &  23    &  1.69  &  2.62  &  9.8   &  V &  \citet{Tempesti1975} \\
    12	  &  1974-08-27.1  &  29    &  1.71  &  2.62  &  12.2  &  V &  \citet{Lustig1976}    \\
    13	  &  1974-08-28.0  &  91    &  1.71  &  2.62  &  12.1  &  V &  \citet{Lustig1976}  \\
    14	  &  1974-08-29.0  &  92    &  1.71  &  2.62  &  11.9  &  V &  \citet{Lustig1976}  \\
    15	  &  1990-08-01.9  &  76    &  1.86  &  2.68  &  15.5  &  V &  \citet{Shevchenko1992} \\
    16	  &  1993-03-21.6  &  77    &  2.55  &  3.47  &  7.6   &  V &  \citet{Michalowski1995b} \\
    17	  &  1993-03-23.6  &  73    &  2.56  &  3.47  &  7.9   &  V &  \citet{Michalowski1995b} \\
    18	  &  1996-12-13.2  &  512   &  1.83  &  2.74  &  9.6   &  V &  \citet{Sato2014}     \\
    19	  &  1996-12-13.3  &  354   &  1.83  &  2.74  &  9.6   &  R &  \citet{Sato2014}     \\
    20	  &  2003-03-31.9  &  29    &  2.85  &  3.20  &  17.8  &  C &  Stephane Charbonnel     \\
    21	  &  2003-03-31.9  &  55    &  2.85  &  3.20  &  17.8  &  C &  Nathanal Berger  \\
    22	  &  2006-06-04.1  &  30    &  2.46  &  2.79  &  21.0  &  C &  Arnaud Leroy     \\
    23	  &  2006-07-21    &  59    &  1.89  &  2.74  &  14.3  &  C &  \citet{Grice2017}     \\
    24	  &  2006-07-25    &  53    &  1.86  &  2.73  &  13.3  &  C &  \citet{Grice2017}  \\
    25	  &  2006-07-25    &  54    &  1.86  &  2.73  &  13.3  &  C &  \citet{Grice2017}  \\
    26	  &  2006-07-26    &  38    &  1.85  &  2.73  &  13.1  &  C &  \citet{Grice2017}\\
    27	  &  2006-07-26    &  40    &  1.85  &  2.73  &  13.1  &  C &  \citet{Grice2017}\\
    28	  &  2006-07-27    &  50    &  1.85  &  2.73  &  12.8  &  C &  \citet{Grice2017}   \\
    29	  &  2006-07-27    &  55    &  1.85  &  2.73  &  12.8  &  C &  \citet{Grice2017}   \\
    30	  &  2006-07-28    &  56    &  1.84  &  2.73  &  12.6  &  C &  \citet{Grice2017}   \\
    31	  &  2006-07-28    &  56    &  1.84  &  2.73  &  12.6  &  C &  \citet{Grice2017}   \\
    32	  &  2006-07-29    &  54    &  1.83  &  2.73  &  12.3  &  C &  \citet{Grice2017}   \\
    33	  &  2006-07-29    &  58    &  1.83  &  2.73  &  12.3  &  C &  \citet{Grice2017}   \\
    34	  &  2006-07-30    &  59    &  1.82  &  2.72  &  12.1  &  C &  \citet{Grice2017}   \\
    35	  &  2006-07-30    &  59    &  1.82  &  2.72  &  12.1  &  C &  \citet{Grice2017}   \\
    36	  &  2006-07-31    &  46    &  1.82  &  2.72  &  11.8  &  C &  \citet{Grice2017}   \\
    37	  &  2006-07-31    &  59    &  1.82  &  2.72  &  11.8  &  C &  \citet{Grice2017}   \\
    38	  &  2006-08-02    &  64    &  1.81  &  2.72  &  11.3  &  C &  \citet{Grice2017}   \\
    39	  &  2006-08-04    &  89    &  1.79  &  2.72  &  10.8  &  C &  \citet{Grice2017}   \\
    40	  &  2006-08-05    &  51    &  1.79  &  2.72  &  10.6  &  C &  \citet{Grice2017}   \\
    41	  &  2006-08-05    &  87    &  1.79  &  2.72  &  10.6  &  C &  \citet{Grice2017}   \\
    42	  &  2006-08-06    &  61    &  1.78  &  2.72  &  10.3  &  C &  \citet{Grice2017}   \\
    43	  &  2006-08-06    &  89    &  1.78  &  2.72  &  10.3  &  C &  \citet{Grice2017}   \\
    44	  &  2006-08-07    &  62    &  1.78  &  2.72  &  10.1  &  C &  \citet{Grice2017}   \\
    45	  &  2006-08-07    &  88    &  1.78  &  2.72  &  10.1  &  C &  \citet{Grice2017}   \\
    46	  &  2006-08-12    &  105   &  1.76  &  2.71  &  9.0   &  C &  \citet{Grice2017}   \\
    47	  &  2006-08-12    &  118   &  1.76  &  2.71  &  9.0   &  C &  \citet{Grice2017}   \\
    48	  &  2006-08-13    &  67    &  1.75  &  2.71  &  8.9   &  C &  \citet{Grice2017}   \\
    49	  &  2006-08-13    &  91    &  1.75  &  2.71  &  8.9   &  C &  \citet{Grice2017}   \\
    50	  &  2006-08-19    &  49    &  1.74  &  2.70  &  8.1   &  C &  \citet{Grice2017}   \\
    51	  &  2006-08-20    &  41    &  1.74  &  2.70  &  8.0   &  C &  \citet{Grice2017}   \\
    52	  &  2006-08-22    &  54    &  1.73  &  2.70  &  7.9   &  C &  \citet{Grice2017}   \\
    53	  &  2006-08-25    &  42    &  1.73  &  2.70  &  8.0   &  C &  \citet{Grice2017}   \\
    54	  &  2006-08-30    &  52    &  1.73  &  2.69  &  8.4   &  C &  \citet{Grice2017}   \\
    55	  &  2006-08-31    &  67    &  1.73  &  2.69  &  8.5   &  C &  \citet{Grice2017}   \\
    56	  &  2006-08-32.0  &  236   &  1.73  &  2.69  &  8.5   &  C &  Dominique Suys, Hugo Riemis, Jan Vantomme\\
    57	  &  2006-09-02    &  52    &  1.74  &  2.69  &  8.9   &  C &  \citet{Grice2017}   \\
    58	  &  2006-09-12    &  57    &  1.77  &  2.68  &  11.1  &  C &  \citet{Grice2017}   \\
    59	  &  2006-09-14    &  50    &  1.77  &  2.68  &  11.6  &  C &  \citet{Grice2017}   \\
    60	  &  2006-09-16    &  46    &  1.78  &  2.68  &  12.1  &  C &  \citet{Grice2017}   \\
    61	  &  2006-09-19    &  38    &  1.80  &  2.67  &  12.9  &  C &  \citet{Grice2017}   \\
    62	  &  2006-09-22    &  46    &  1.82  &  2.67  &  13.7  &  C &  \citet{Grice2017}   \\
    63	  &  2006-09-24    &  47    &  1.83  &  2.67  &  14.3  &  C &  \citet{Grice2017}   \\
    64	  &  2006-09-26    &  47    &  1.84  &  2.67  &  14.8  &  C &  \citet{Grice2017}   \\
    65	  &  2006-09-27    &  38    &  1.85  &  2.67  &  15.0  &  C &  \citet{Grice2017}   \\
    66	  &  2006-10-08    &  43    &  1.94  &  2.66  &  17.6  &  C &  \citet{Grice2017}   \\
    67	  &  2007-10-18    &  39    &  2.29  &  2.78  &  19.8  &  C &  \citet{Grice2017}   \\
    68	  &  2007-11-22    &  80    &  1.96  &  2.82  &  11.7  &  C &  \citet{Grice2017}   \\
    69	  &  2007-12-27.9  &  34    &  1.90  &  2.87  &  3.1   &  C &  Jean-Francois Coliac    \\
    70	  &  2008-12-28    &  58    &  2.94  &  3.37  &  16.2  &  C &  \citet{Grice2017}   \\
    71	  &  2009-01-03    &  59    &  2.87  &  3.37  &  15.5  &  C &  \citet{Grice2017}   \\
    72	  &  2009-01-04    &  58    &  2.85  &  3.38  &  15.4  &  C &  \citet{Grice2017}   \\
    73	  &  2009-01-17    &  61    &  2.71  &  3.39  &  13.5  &  C &  \citet{Grice2017}   \\
    74	  &  2009-01-18    &  55    &  2.70  &  3.39  &  13.4  &  C &  \citet{Grice2017}   \\
    75	  &  2009-01-20    &  53    &  2.68  &  3.39  &  13.0  &  C &  \citet{Grice2017}   \\
    76	  &  2009-01-20    &  73    &  2.68  &  3.39  &  13.0  &  C &  \citet{Grice2017}   \\
    77	  &  2009-01-21    &  58    &  2.67  &  3.39  &  12.8  &  C &  \citet{Grice2017}   \\
    78	  &  2009-01-23    &  51    &  2.65  &  3.39  &  12.4  &  C &  \citet{Grice2017}   \\
    79	  &  2009-01-24    &  55    &  2.65  &  3.39  &  12.2  &  C &  \citet{Grice2017}   \\
    80	  &  2009-01-24    &  77    &  2.64  &  3.39  &  12.2  &  C &  \citet{Grice2017}   \\
    81	  &  2009-01-25    &  56    &  2.64  &  3.40  &  12.0  &  C &  \citet{Grice2017}   \\
    82	  &  2009-01-26    &  61    &  2.63  &  3.40  &  11.8  &  C &  \citet{Grice2017}   \\
    83	  &  2009-01-27    &  71    &  2.62  &  3.40  &  11.6  &  C &  \citet{Grice2017}   \\
    84	  &  2009-01-28    &  73    &  2.61  &  3.40  &  11.4  &  C &  \citet{Grice2017}   \\
    85	  &  2009-01-31    &  60    &  2.59  &  3.40  &  10.8  &  C &  \citet{Grice2017}   \\
    86	  &  2009-02-01    &  37    &  2.58  &  3.40  &  10.6  &  C &  \citet{Grice2017}   \\
    87	  &  2009-02-02    &  77    &  2.58  &  3.40  &  10.4  &  C &  \citet{Grice2017}   \\
    88	  &  2009-02-16    &  46    &  2.50  &  3.42  &  7.5   &  C &  \citet{Grice2017}   \\
    89	  &  2009-02-18    &  85    &  2.50  &  3.42  &  7.1   &  C &  \citet{Grice2017}   \\
    90	  &  2009-02-19    &  46    &  2.49  &  3.42  &  7.0   &  C &  \citet{Grice2017}   \\
    91	  &  2009-02-21    &  81    &  2.49  &  3.42  &  6.7   &  C &  \citet{Grice2017}   \\
    92	  &  2009-02-21    &  84    &  2.49  &  3.42  &  6.7   &  C &  \citet{Grice2017}   \\
    93	  &  2009-02-22    &  47    &  2.49  &  3.42  &  6.6   &  C &  \citet{Grice2017}   \\
    94	  &  2009-02-22    &  63    &  2.49  &  3.42  &  6.6   &  C &  \citet{Grice2017}   \\
    95	  &  2009-02-26    &  40    &  2.48  &  3.42  &  6.2   &  C &  \citet{Grice2017}   \\
    96	  &  2009-02-27    &  48    &  2.48  &  3.42  &  6.1   &  C &  \citet{Grice2017}   \\
    97	  &  2009-03-01    &  50    &  2.48  &  3.43  &  6.1   &  C &  \citet{Grice2017}   \\
    98	  &  2009-03-02    &  83    &  2.48  &  3.43  &  6.1   &  C &  \citet{Grice2017}   \\
    99	  &  2009-03-04    &  55    &  2.49  &  3.43  &  6.1   &  C &  \citet{Grice2017}   \\
   100	  &  2009-03-13    &  93    &  2.51  &  3.44  &  7.0   &  C &  \citet{Grice2017}   \\
   101	  &  2009-03-14    &  65    &  2.51  &  3.44  &  7.2   &  C &  \citet{Grice2017}   \\
   102	  &  2009-03-16    &  53    &  2.52  &  3.44  &  7.6   &  C &  \citet{Grice2017}   \\
   103	  &  2009-03-17    &  61    &  2.53  &  3.44  &  7.7   &  C &  \citet{Grice2017}   \\
   104	  &  2009-03-19    &  64    &  2.54  &  3.44  &  8.1   &  C &  \citet{Grice2017}   \\
   105	  &  2009-03-20    &  47    &  2.54  &  3.44  &  8.3   &  C &  \citet{Grice2017}   \\
   106	  &  2009-03-20    &  79    &  2.54  &  3.44  &  8.3   &  C &  \citet{Grice2017}   \\
   107	  &  2009-03-21    &  42    &  2.55  &  3.44  &  8.5   &  C &  \citet{Grice2017}   \\
   108	  &  2009-03-21    &  71    &  2.55  &  3.44  &  8.5   &  C &  \citet{Grice2017}   \\
   109	  &  2009-03-22    &  49    &  2.55  &  3.44  &  8.8   &  C &  \citet{Grice2017}   \\
   110	  &  2009-03-22    &  76    &  2.55  &  3.44  &  8.7   &  C &  \citet{Grice2017}   \\
   111	  &  2009-03-23    &  65    &  2.56  &  3.44  &  8.9   &  C &  \citet{Grice2017}   \\
   112	  &  2009-03-28    &  85    &  2.59  &  3.45  &  10.0  &  C &  \citet{Grice2017}   \\
   113	  &  2009-03-29    &  83    &  2.60  &  3.45  &  10.2  &  C &  \citet{Grice2017}   \\
   114	  &  2009-03-30    &  36    &  2.61  &  3.45  &  10.4  &  C &  \citet{Grice2017}   \\
   115	  &  2009-03-30    &  74    &  2.61  &  3.45  &  10.4  &  C &  \citet{Grice2017}   \\
   116	  &  2009-03-30    &  77    &  2.61  &  3.45  &  10.4  &  C &  \citet{Grice2017}   \\
   117	  &  2009-03-31    &  52    &  2.62  &  3.45  &  10.6  &  C &  \citet{Grice2017}   \\
   118	  &  2009-04-01    &  75    &  2.63  &  3.45  &  10.8  &  C &  \citet{Grice2017}   \\
   119	  &  2009-04-01    &  77    &  2.63  &  3.45  &  10.8  &  C &  \citet{Grice2017}   \\
   120	  &  2009-04-02    &  75    &  2.64  &  3.45  &  11.0  &  C &  \citet{Grice2017}   \\
   121	  &  2009-04-12    &  71    &  2.73  &  3.46  &  12.9  &  C &  \citet{Grice2017}   \\
   122	  &  2009-05-12    &  35    &  3.11  &  3.48  &  16.5  &  C &  \citet{Grice2017}   \\
   123	  &  2009-05-12    &  35    &  3.11  &  3.48  &  16.5  &  C &  \citet{Grice2017}   \\
   124	  &  2011-06-02    &  51    &  2.23  &  2.98  &  15.2  &  C &  \citet{Grice2017}   \\
   125	  &  2011-06-12    &  50    &  2.12  &  2.97  &  12.8  &  C &  \citet{Grice2017}   \\
   126	  &  2011-06-12    &  62    &  2.12  &  2.97  &  12.8  &  C &  \citet{Grice2017}   \\
   127	  &  2011-06-13    &  57    &  2.11  &  2.97  &  12.5  &  C &  \citet{Grice2017}   \\
   128	  &  2011-06-13    &  74    &  2.11  &  2.97  &  12.5  &  C &  \citet{Grice2017}   \\
   129	  &  2011-06-20    &  41    &  2.04  &  2.96  &  10.4  &  C &  \citet{Grice2017}   \\
   130	  &  2011-06-21    &  40    &  2.03  &  2.95  &  10.1  &  C &  \citet{Grice2017}   \\
   131	  &  2011-07-08    &  39    &  1.93  &  2.93  &  4.5   &  C &  \citet{Grice2017}   \\
   132	  &  2011-07-09    &  47    &  1.93  &  2.93  &  4.1   &  C &  \citet{Grice2017}   \\
   133	  &  2011-07-09    &  69    &  1.93  &  2.93  &  4.2   &  C &  \citet{Grice2017}   \\
   134	  &  2011-07-10    &  41    &  1.92  &  2.93  &  3.8   &  C &  \citet{Grice2017}   \\
   135	  &  2011-07-10    &  79    &  1.92  &  2.93  &  3.8   &  C &  \citet{Grice2017}   \\
   136	  &  2011-07-18    &  41    &  1.90  &  2.91  &  2.5   &  C &  \citet{Grice2017}   \\
   137	  &  2011-07-31    &  39    &  1.91  &  2.89  &  6.0   &  C &  \citet{Grice2017}   \\
   138	  &  2011-08-01    &  39    &  1.91  &  2.89  &  6.4   &  C &  \citet{Grice2017}   \\
   139	  &  2011-08-06    &  45    &  1.93  &  2.89  &  8.1   &  C &  \citet{Grice2017}   \\
   140	  &  2012-09-17.0  &  151   &  2.05  &  2.62  &  20.6  &  C &  K. Sobkowiak, Borowiec, Poland    \\
   141	  &  2012-09-18.9  &  17    &  2.03  &  2.62  &  20.3  &  C &  J. Nadolny, Borowiec, Poland    \\
   142	  &  2012-09-24.0  &  10    &  1.98  &  2.62  &  19.4  &  C &  J. Nadolny, Borowiec, Poland    \\
   143	  &  2012-10-01.0  &  83    &  1.91  &  2.63  &  18.1  &  C &  M. Bronikowska, Borowiec, Poland    \\
   144	  &  2012-11-29.9  &  45    &  1.75  &  2.67  &  9.3   &  C &  Francisco Soldan \\
   145	  &  2012-12-01.9  &  48    &  1.76  &  2.67  &  9.8   &  C &  Francisco Soldan \\
   146	  &  2012-12-02.9  &  59    &  1.77  &  2.68  &  10.1  &  C &  Francisco Soldan \\
   147	  &  2012-12-08.9  &  29    &  1.81  &  2.68  &  11.7  &  C &  Francisco Soldan \\
   148	  &  2012-12-26.0  &  18    &  1.96  &  2.70  &  16.1  &  C &  Francisco Soldan \\
   149	  &  2012-12-26.0  &  24    &  1.96  &  2.70  &  16.1  &  C &  Francisco Soldan \\
   150	  &  2012-12-26.8  &  174   &  1.97  &  2.70  &  16.3  &  C &  Francisco Soldan \\
   151	  &  2012-12-27.8  &  145   &  1.98  &  2.70  &  16.6  &  C &  Francisco Soldan \\
   152	  &  2012-12-28.8  &  23    &  1.99  &  2.70  &  16.8  &  C &  Francisco Soldan \\
   153	  &  2012-12-28.8  &  55    &  1.99  &  2.70  &  16.8  &  C &  Francisco Soldan \\
   154	  &  2016-05-23.1  &  52    &  2.27  &  3.18  &  9.3   &  C &  Raul Melia, Cordoba, Argentina     \\
   155	  &  2016-06-15.1  &  52    &  2.14  &  3.15  &  2.3   &  C &  Carlos Colazo, Cordoba, Argentina     \\
   156	  &  2016-06-16.2  &  42    &  2.14  &  3.15  &  2.1   &  C &  Carlos Colazo, Cordoba, Argentina    \\
   157	  &  2016-07-25.9  &  51    &  2.26  &  3.09  &  12.9  &  C &  A. Marciniak, Obs. del Teide, Spain   \\
   158	  &  2017-07-16.4  &  149   &  2.22  &  2.62  &  22.3  &  V &  \citet{Warner2018}     \\
   159	  &  2017-07-17.4  &  172   &  2.21  &  2.62  &  22.2  &  V &  \citet{Warner2018}    \\
   160	  &  2017-07-18.4  &  156   &  2.20  &  2.62  &  22.2  &  V &  \citet{Warner2018}    \\
   161	  &  2017-07-21.4  &  201   &  2.16  &  2.62  &  22.0  &  V &  \citet{Warner2018}  \\
   162	  &  2017-07-22.4  &  196   &  2.15  &  2.62  &  21.9  &  V &  \citet{Warner2018}  \\
   163	  &  2017-07-23.0  &  29    &  2.14  &  2.62  &  21.8  &  r' & R. Szakats, Piszkes Obs., Hungary     \\
   164	  &  2017-08-01.0  &  47    &  2.04  &  2.61  &  20.9  &  C &  Adrian Jones, Gaia-GOSA \\
   165	  &  2017-08-12.0  &  23    &  1.93  &  2.61  &  19.3  &  R &  R. Szakats, Piszkes Obs., Hungary\\
   166	  &  2017-08-14.0  &  35    &  1.91  &  2.61  &  19.0  &  R &  R. Szakats, Piszkes Obs., Hungary    \\
   167	  &  2017-08-15.1  &  17    &  1.90  &  2.60  &  18.8  &  R &  R. Szakats, Piszkes Obs., Hungary     \\
   168	  &  2017-08-16.0  &  66    &  1.89  &  2.60  &  18.6  &  R &  R. Szakats, Piszkes Obs., Hungary     \\
   169	  &  2017-10-11.9  &  38    &  1.67  &  2.59  &  11.1  &  r' & R. Szakats, Piszkes Obs., Hungary  \\
   170	  &  2017-10-16.8  &  139   &  1.69  &  2.59  &  11.8  &  R &  R. Duffard, La Sagra, Spain     \\
   171	  &  2017-11-08.9  &  154   &  1.83  &  2.59  &  16.8  &  R &  R. Duffard, La Sagra, Spain     \\
   172	  &  2017-11-15.9  &  276   &  1.89  &  2.59  &  18.2  &  R &  R. Duffard, La Sagra, Spain     \\
   173	  &  2017-11-16.9  &  188   &  1.90  &  2.59  &  18.4  &  R &  R. Duffard, La Sagra, Spain     \\
   174	  &  2017-12-4.0   &  76    &  2.07  &  2.59  &  20.9  &  C &  D. Molina, Gaia-GOSA    \\
   175	  &  2017-7-14.1   &  58    &  2.25  &  2.62  &  22.4  &  C &  D. Molina, Gaia-GOSA    \\
   176	  &  2017-7-16.2   &  63    &  2.22  &  2.62  &  22.3  &  C &  D. Molina, Gaia-GOSA    \\
   177	  &  2017-7-23.2   &  48    &  2.14  &  2.62  &  21.8  &  C &  D. Molina, Gaia-GOSA    \\
   178	  &  2017-7-26.2   &  35    &  2.11  &  2.62  &  21.6  &  C &  D. Molina, Gaia-GOSA    \\
   179	  &  2017-7-27.2   &  58    &  2.10  &  2.62  &  21.5  &  C &  D. Molina, Gaia-GOSA    \\
   180	  &  2017-8-6.1    &  187   &  1.99  &  2.61  &  20.3  &  C &  A. Jones, Gaia-GOSA    \\
   181	  &  2018-12-09.1  &  83    &  2.22  &  3.01  &  13.2  &  V &  C. Garcia, Gaia-GOSA \\
   182	  &  2018-12-10.1  &  100   &  2.21  &  3.01  &  13.0  &  V &  C. Garcia, Gaia-GOSA \\
   183	  &  2018-12-14.0  &  54    &  2.18  &  3.01  &  11.8  &  V &  C. Garcia, Gaia-GOSA \\
   184	  &  2018-12-3.3   &  1395  &  2.28  &  3.00  &  14.8  & Rc &  E. Jehin, M. Ferrais, TRAPPIST-N and -S \\
   185	  &  2019-1-16.2   &  540   &  2.09  &  3.06  &  2.1   & Rc &  E. Jehin, M. Ferrais, TRAPPIST-S \\
   186	  &  2019-1-19.2   &  492   &  2.09  &  3.07  &  2.7   & Rc &  E. Jehin, M. Ferrais, TRAPPIST-S \\
   187	  &  2019-1-26.3   &  811   &  2.12  &  3.08  &  4.9   & Rc &  E. Jehin, M. Ferrais, TRAPPIST-S \\
   188	  &  2019-2-1.2    &  269   &  2.16  &  3.09  &  7.0   & Rc &  E. Jehin, M. Ferrais, TRAPPIST-S \\
   189	  &  2019-1-16.1   &  269   &  2.09  &  3.06  &  2.1   & r' &  M. Person, T. Brothers\\
   190    &  2012-12 -- 2018-1 & 198&        &        &        & V  &  ASAS-SN \\
   191    &  2015-1 -- 2016-4  & 16 &        &        &        & V  &  Gaia DR2 \\
   \hline
\end{longtable}
\tablefoot{
     Gaia-GOSA (Gaia-Ground-based Observational Service for Asteroids, \url{www.gaiagosa.eu}).
    }



==> tabs/tab_mass2.tex <==
\begin{table*}[h]
\begin{center}
  \caption[Mass estimates of (704) Interamnia]{
    The mass estimates ($\mathcal{M}$) of (704) Interamnia collected in the literature. For each, the 1\,$\sigma$ uncertainty, method, selection flag, and bibliographic reference are reported. The methods are \textsc{defl}: Deflection, \textsc{ephem}: Ephemeris. \label{tab:mass}}
  \begin{tabular}{rrlcl}
    \hline\hline
     \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{Mass ($\mathcal{M}$)} &

     \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{Sel.} & \multicolumn{1}{c}{Reference}  \\
    & \multicolumn{1}{c}{(kg)} \\
    \hline
  1 & $(7.36 \pm 3.38) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{Landgraf1992}           \\
  2 & $12.3_{-12.3}^{+13.1} \times 10^{19}$              & \textsc{defl}  & \ding{55} & \citet{1999-IAA-Vasiliev}                \\
  3 & $(2.59 \pm 0.14) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2001-IAA-Krasinsky}               \\
  4 & $(7.00 \pm 1.85) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{Michalak2001}             \\
  5 & $(1.61 \pm 0.84) \times 10^{19}$                  & \textsc{defl}  & \ding{55} & \citet{2002-ACM-Chernetenko}             \\
  6 & $(1.61 \pm 0.84) \times 10^{19}$                  & \textsc{defl}  & \ding{55} & \citet{2004-SoSyR-38-Kochetova}          \\
  7 & $(7.12 \pm 0.84) \times 10^{19}$                   & \textsc{defl}  & \ding{55} & \citet{Baer2008}              \\
  8 & $(11.30 \pm 3.18) \times 10^{19}$                  & \textsc{defl}  & \ding{55} & \citet{2008-PSS-56-Ivantsov}             \\
  9 & $(3.23 \pm 0.02) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{Fienga2009}               \\
 10 & $(3.69 \pm 0.37) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2009-SciNote-Folkner}             \\
 11 & $(2.66 \pm 1.09) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{Somenzi2010}              \\
 12 & $(3.88 \pm 0.18) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2011-AJ-141-Baer}                 \\
 13 & $(3.97 \pm 1.31) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2011-Icarus-211-Konopliv}         \\
 14 & $(2.25 \pm 0.66) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2011-AJ-142-Zielenbach}           \\
 15 & $(3.34 \pm 0.52) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2011-AJ-142-Zielenbach}           \\
 16 & $(3.13 \pm 0.52) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2011-AJ-142-Zielenbach}           \\
 17 & $(3.88 \pm 0.75) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2011-AJ-142-Zielenbach}           \\
 18 & $(3.82 \pm 0.36) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2011-DPS-Fienga}                  \\
 19 & $(3.82 \pm 0.47) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2012-SciNote-Fienga}              \\
 20 & $(3.94 \pm 0.69) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2013-Icarus-222-Kuchynka}         \\
 21 & $(2.43 \pm 0.19) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2013-SoSyR-47-Pitjeva}            \\
 22 & $(3.82 \pm 0.41) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2014-SciNote-Fienga}              \\
 23 & $(2.72 \pm 0.12) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2014-AA-565-Goffin}               \\
 24 & $(3.42 \pm 0.18) \times 10^{19}$                   & \textsc{defl}  & \ding{51} & \citet{2014-SoSyR-48-Kochetova}          \\
 25 & $(4.18 \pm 0.44) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2017-BDL-108-Viswanathan}         \\
 26 & $0.31_{-0.31}^{0.80} \times 10^{19}$              & \textsc{defl}  & \ding{55} & \citet{2017-Icarus-297-Siltala}          \\
 27 & $(4.38 \pm 0.24) \times 10^{19}$                   & \textsc{ephem} & \ding{51} & \citet{2017-AJ-154-Baer}                 \\
\hline
 & $(3.79 \pm 1.28) \times 10^{19}$ & \multicolumn{2}{c}{Average} \\
   \hline
  \end{tabular}
\end{center}
\end{table*}


==> tabs/tab_occ.tex <==
\onecolumn
%\twocolumn
%\begin{multicols}{2}
%\shortlipsum
%\medskip
%\scriptsize{
%\longtab{2}{
%\begin{tabular}{r@{\,\,\,}l lc| r@{\,\,\,}l lc} \hline
% \multicolumn{2}{c} {Asteroid} & Date & Observer &  \multicolumn{2}{c}{Asteroid} & Date & Observer\\ \hline\hline
\begin{longtable}{l}
\caption{\label{tab:occ}List of stellar occultations used for shape modeling, with individual observers names.}\\
\hline
\multicolumn{1}{c} {\textbf{(704) Interamnia}} \\ \hline\hline

\endfirsthead
\caption{continued.}\\

\hline
 Observer \\ \hline\hline
\endhead
\hline
\endfoot
\multicolumn{1}{c} {\textbf{1996-12-17}} \\
Bob Fried, Braeside Obs.,Flagstaff, AZ, USA \\
Gary Goodman, Camarillo, CA, USA           \\
Etscorn Obs., Socorro, NM, USA             \\
Orange County A.S. Obs., Anza, CA, USA\\
F. Wright/Fulton Jr., Prescott, AZ, USA \\
Pierre Schwaar, Phoenix, AZ, USA    \\
P. Maley/L Paller, Phoenix, AZ, USA    \\
Sam Herchak, Mesa, AZ, USA         \\
Table Mtn. Obs., Wrightwood, CA, USA   \\
Ken Ziegler, Gila Obs., Globe, AZ, USA \\
Bill Peters, AZ, USA                   \\ \hline
\multicolumn{1}{c} {\textbf{2003-3-23}} \\
Yoshida Hidetoshi, Abashiri, Hokkaido, JP \\
Kouda Masaki, Kamikita, Aomori, JP    \\
Imatani \& Takashi, Kitaura, Ibaraka, JP \\
Sugawara Hitoshi, Ichinoseki, Iwate, JP \\
Satou Toshirou, Ichinoseki, Iwate, JP \\
Yokokawa Mikio, Motoyoshi, Miyagi, JP \\
Konno Eitoshi, Hanaizumi, Iwate JP    \\
Sasaki Kazuo, Furukawa, Miyagi, JP    \\
Tonomura Yasuhiro, Tomiya, Miyagi, JP \\
Okamoto Michiko, Rifu, Miyagi, JP     \\
Sakaki Chiyoaki, Sendai, Miyagi, JP   \\
Nagai Hideo, Sendai, Miyagi, JP       \\
Itou Yoshiharu, Aoba, Sendai, JP      \\
Ikeshita Ryo et al., Kawauchi, Sendai, JP \\
Koishikawa Masahiro, Sendai, Miyagi, JP \\
Watanabe, Akira, Sendai, Miyagi, JP   \\
Miyamoto Atsushi et al, Adachi, JP    \\
Sugai Hideo, Zao-hango, Yamagata, JP  \\
Fujita Mitsuhiro, Shiroishi, Miyagi, JP \\
Nihei Hajime, Nanyo, Yamagata, JP     \\
Tanaka Takashi, Zushi, Kanagawa, JP    \\
Sato Tsutomu, Marumori, Miyagi, JP    \\
Ootsuki Isao, Marumori, Miyagi, JP    \\
David Tholen, Turtle Bay, Oahu, Hawaii, USA \\
Sato Hikaru, Fukushima, JP            \\
Sato Makoto, Haranomachi, Fukushima, JP \\
Rebecca Sydney, Honolua Bay, Maui, HI \\
Bedient et al., Foster Village, Hawaii, USA \\
Hamanowa et al., Koriyama City, JP     \\
Usuki Ken-ichi, Niitsuru, Fukushima, JP \\
Lewis Roberts, Haleakala, Hawaii, USA  \\
Watanabe et al., Takine, Fukushima, JP \\
Sato Hirohisa, Sukagawa, Fukushima, JP \\
David Dunham, Makena, Maui, HI, USA    \\
B. Brevoort, Hawaii, USA                \\
Tsuchikawa Akira, Yanagida, JP        \\
S. Bus, Mauna Kea, Hawaii, USA         \\
R. Savalle, Mauna Kea, Hawaii, USA     \\
Tomioka Hiroyuki, Hitachi, Ibaraki, JP \\
P. Maley, Hawaii, USA                  \\
Yaeza Akira,Moriyama-cho, Hitachi, JP  \\
E. Cleintuar, Hawaii, USA              \\
S. O'Meara, Mauna Loa, USA             \\
W. Fukunaga, Hawaii, USA               \\
V. Fukunaga, Hawaii, USA               \\
J. Swatek, Hawaii, USA                 \\
Uehara Sadaharu, Ibaraki, JP          \\
Kuboniwa Atasushi, Ushika,Ibaraka, JP \\
Kita Nobusuke, Kashiwa, Chiba, JP     \\
Takashima et al, Kashiwa, Chiba, JP   \\
Momose Masahiko, Shiojiri, Nagano, JP \\
Kaneko Sakae, Sakura, Chiba, JP       \\
Nakanishi Akio, Itabashi, Tokyo, JP   \\
Ishida Masayuki, Kanazu, Fukui, JP    \\
Kitazaki Katsuhiko, Tokyo, JP         \\
Ida Miyoshi, Muraoka, Fukui, JP       \\
Suzuki Satoshi, Yokohama,Kanagawa, JP \\
Hirose Yoji, Chigasaki, Kanagawa, JP  \\
Sugiyama Yukihiro, Hiratsuka, JP      \\
Yoneyama Seiichi, Ogaki, Gifu, JP     \\
Oribe Takaaki et al., Saji, Tottori, JP \\ \hline
\multicolumn{1}{c} {\textbf{2007-9-9}} \\
R. Cadmus, Grinnell, IA, USA          \\
J. Centala, Marion, IA, USA            \\
W. Osborn/C. Tycner, Mt. Pleasant, MI, USA\\
P. Maley, Bernalillo, NM, USA          \\
K. McKeown, Los Lunas, NM, USA          \\
D. Dunham, Dubuque IA, USA             \\
\multicolumn{1}{c} {\textbf{2012-11-12}} \\ \hline
N. Smith, Trenton, GA, USA               \\
T. Blank/M. Pacht, Taftsville, VT, USA   \\
S. Conard, Gamber, MD, USA            \\
A. Scheck, Scaggsville, MD, USA        \\
C. Ellington, Owings, MD, USA           \\
\hline
 \end{longtable}
%\tablefoot{
%\tablefoottext{a}{On line at \texttt{http://www.david-higgins.com/Astronomy/asteroid/lightcurves.htm}} %Higgins
%}
%}
%}
%\end{multicols}
